Conditional Generation with a Question-Answering Blueprint

The ability to convey relevant and faithful information is critical for many tasks in conditional generation and yet remains elusive for neural seq-to-seq models whose outputs often reveal hallucinations and fail to correctly cover important details. In this work, we advocate planning as a useful intermediate representation for rendering conditional generation less opaque and more grounded. Our work proposes a new conceptualization of text plans as a sequence of question-answer (QA) pairs. We enhance existing datasets (e.g., for summarization) with a QA blueprint operating as a proxy for both content selection (i.e.,~what to say) and planning (i.e.,~in what order). We obtain blueprints automatically by exploiting state-of-the-art question generation technology and convert input-output pairs into input-blueprint-output tuples. We develop Transformer-based models, each varying in how they incorporate the blueprint in the generated output (e.g., as a global plan or iteratively). Evaluation across metrics and datasets demonstrates that blueprint models are more factual than alternatives which do not resort to planning and allow tighter control of the generation output.

==> tables/aquamuse-results.tex <==

\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1}
\small
\begin{tabular}{l | c c c c c | c c c}
\toprule
\multirow{3}{*}{\textbf{System (xl)}} & \multicolumn{5}{c}{\textbf{Evaluating Summary}} & \multicolumn{3}{c}{\textbf{Evaluating Blueprint}}  \\
& \multicolumn{3}{c}{\textbf{Rouge}} & \textbf{Faithfulness}  & \textbf{Grounding} & \multicolumn{3}{c}{\textbf{Rouge}} \\
& R1 & R2 & RL & acc.(conf.) & F1 & R1 & R2 & RL \\ \midrule 
\tv & 44.93 & 27.10 & 41.53 & 70.01 (66.13) & & -- & -- & -- \\
% LongT5 (4096x256) & 60.64 & 45.99 & 57.81 & 74.52 & 79.44 \\
\longtv & 64.11 & 50.60 & 61.43 & 82.52 (77.35) &  & -- & -- & --  \\
\etoe & 61.65 & 48.17 & 58.96 & 83.64 (78.26) & & 57.53 & 34.59 & 54.16  \\
\aplan & 61.91 & 48.45 & 59.24 &  83.37 (77.88) & & 57.96 & 34.77 & 54.88 \\
\iterative & 59.25 & 45.07 & 56.48 & 84.77 (79.07) & & 55.79 & 32.87 & 52.92  \\
\midrule
\etoe-filtered & 61.43 & 48.18 & 58.74 & 83.98 (78.81) &  & 56.08 & 33.72 & 52.71\\
\aplan-filtered & 61.97 & 48.48 & 59.25 & 84.98 (79.20) &  & 57.01 & 33.90 & 53.79 \\
\iterative-filtered & 59.09 & 44.85 & 56.30 & 85.50 (79.78) & & 56.03 & 32.51 & 52.83 \\
% 59.09 & 44.85 & 56.30 & 85.50 (79.78) & \\
\iterative-Q1 & 60.05 & 47.11 & 57.41 & 86.79 (81.66) &  & 40.76 & 21.82 & 37.30 \\
\bottomrule
\end{tabular}
\caption{Aquamuse results on the test set. \sn{Evaluate Plans and Groundedness automatically}}
\end{table*}



==> tables/human-eval-results.tex <==
\begin{table}[t!]
\center
% \scriptsize
%\tiny
\resizebox{\linewidth}{!}{
{\setlength{\tabcolsep}{0pt}%
\begin{tabular}{l@{}|@{~} c|@{~} c@{~~} c @{~}|@{~} c@{~~} c@{~~} c@{}} \hline
& summary & \multicolumn{2}{c@{~}|@{~}}{blueprint} &  \multicolumn{3}{c@{~}@{~}}{grounding} \\
% & \multicolumn{2}{c@{~}|@{~}}{Rouge (RLSum)} &  \multicolumn{2}{c|@{~}}{QA-F1} & \multicolumn{1}{c}{ANLI}  \\ 
& best & quality & redund.& abs. & contr. & new-info \\ 
Models & 0-to-1 & 1-to-3 & \% & \% & \% & 3-to-1 \\ \hline 
\textsc{r2t-Bart} & 0.10 & --- & --- & --- & --- & \multicolumn{1}{c}{---}  \\  
\longtv & 0.42$^{\diamond\dagger\ddagger}$ & --- & --- & --- & --- & \multicolumn{1}{c}{---}  \\  
\cellcolor{DarkBP}\textcolor{black}{\etoe} & 0.26 & \textbf{2.43} & 49.3 & 26.6 & 5.3$^\diamond$ & 1.76$^\diamond$ \\
\cellcolor{DarkBP}\textcolor{black}{\aplan} & 0.39$^{\diamond\ast}$ & 2.28$^\diamond$ & \textbf{33.0} & 63.0 & 8.7  & 2.60 \\
\cellcolor{DarkBP}\textcolor{black}{\iterative} & \textbf{0.44}$^\dagger$ & 2.09 & 81.7 & \textbf{12.0}$^\diamond$ & \textbf{2.8}$^{\dagger}$ & \textbf{1.53} \\
\hspace{0.2cm} \cellcolor{MidBP}\textcolor{black}{+drop} & 0.39$^{\ddagger\ast}$ & 2.28$^\diamond$  & 63.7 & 14.2$^\diamond$ & 3.6$^{\diamond\dagger}$ & 1.89$^\diamond$ \\
\hline
% Gold & --- & 2.02 & 95.7 & 4.5 & 3.9 & 1.39  \\ \hline
\end{tabular}}
}
  \vspace{-0.2cm}
\caption{Human evaluation results on SummScreen-FD recap generation. The best results for each task are \textbf{boldfaced}. 
Systems in each column are marked with same symbols when differences among them are not significant (using a one-way ANOVA with post-hoc Tukey HSD tests; $p < 0.01$).    \label{table:heval-results} }
    \vspace{-0.6cm}
\end{table}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master:  "main"
%%% End:


==> tables/summscreen-fd-results.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1}
\small
\begin{tabular}{l | c c c c c | c c c}
\toprule
\multirow{3}{*}{\textbf{System (xl)}} & \multicolumn{5}{c}{\textbf{Evaluating Summary}} & \multicolumn{3}{c}{\textbf{Evaluating Blueprint}}  \\
& \multicolumn{3}{c}{\textbf{Rouge}} & \textbf{Faithfulness}  & \textbf{Grounding} & \multicolumn{3}{c}{\textbf{Rouge}} \\
& R1 & R2 & RL & acc.(conf.) & F1 & R1 & R2 & RL \\ \midrule 
\tv & 29.92 & 6.58 & 25.84 & 0.78 (2.12) &  & -- & -- & --  \\
% LongT5 (4096x256) &  \\
\longtv & 35.99 & 9.71 & 31.22 & 8.40 (11.19) &  & -- & -- & --   \\
\etoe & 32.63 & 8.19 & 28.22 & 8.53 (11.19) &  & 35.06 & 17.09 & 34.49\\
\aplan & 36.45 & 9.37 & 31.88 & 9.57 (12.49) & & 35.90 & 17.21 & 35.23 \\
\iterative & 33.64 & 8.25 & 29.86 & 20.84 (23.40) &  & 40.09 & 19.25 & 39.36\\
\midrule
\etoe-filtered &  29.55 & 6.73 & 25.50 & 10.00 (13.28) & & 23.61 & 11.85 & 23.22\\
\aplan-filtered &  34.34 & 8.48 & 30.40 & 12.23 (15.43) & & 25.21 & 12.06 & 24.75  \\
\iterative-filtered  & 31.67 & 7.03 & 28.10  & 24.12 (26.06) & & 32.84 & 16.03 & 32.25  \\
\iterative-Q1 & 32.83 & 7.69 & 29.13 & 21.17 (23.66) & & 27.00 & 13.01 & 26.48 \\
\bottomrule
\end{tabular}
\caption{SummScreen-fd results on the test set.}
\end{table*}



==> tables/wikicatsum-results.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1}
\small
\begin{tabular}{l | c c c c c | c c c}
\toprule
\multirow{3}{*}{\textbf{System (xl)}} & \multicolumn{5}{c}{\textbf{Evaluating Summary}} & \multicolumn{3}{c}{\textbf{Evaluating Blueprint}}  \\
& \multicolumn{3}{c}{\textbf{Rouge}} & \textbf{Faithfulness}  & \textbf{Grounding} & \multicolumn{3}{c}{\textbf{Rouge}} \\
& R1 & R2 & RL & acc.(conf.) & F1 & R1 & R2 & RL \\ \midrule 
\tv & 42.44 & 26.22 & 40.17 & 46.21 (44.86) &  & -- & -- & --  \\
% LongT5 (4096x256) &  44.57 & 27.37 & 42.00 & 52.86 &  \\
\longtv & 43.43 & 26.80 & 41.00 & 56.11 (53.15) &  & -- & -- & --  \\
\etoe & 42.03 & 26.35 & 39.78  &  60.56 (57.75) &  & 47.91 & 29.00 & 45.40 \\
\aplan & 44.85 & 27.43 & 42.34 & 52.09 (50.22) & & 49.33 & 29.32 & 46.95  \\
\iterative & 41.95 & 24.34 & 39.53 & 64.37 (61.08) & & 48.84 & 27.50 & 46.35 \\
\midrule
\etoe-filtered & 39.46 & 24.79 & 37.35 & 64.38 (61.10) & & 38.14 & 22.28 & 36.00 \\
\aplan-filtered & 42.99 & 26.14 & 40.65 & 56.71 (54.24) &  & 38.52 & 21.63 & 36.45 \\
\iterative-filtered & 41.19 & 23.61 & 38.80 & 66.56 (62.99) & & 44.30 & 23.86 & 41.78 \\
% 41.19 & 23.61 & 38.80 & 66.56 (62.99) \\
\iterative-Q1 & 40.15 & 25.73 & 38.24 & 65.11 (61.68) & & 34.02 & 16.28 & 31.06 \\

\bottomrule
\end{tabular}
\caption{WikiCatSum results on the test set. \sn{Update Blueprint ROUGE.}} 
\end{table*}


